Gribov process advected by the synthetic compressible velocity ensemble: Renormalization Group Approach

The direct bond percolation process (Gribov process) is studied in the presence of irrotational velocity fluctuations with long-range correlations. The perturbative renormalization group is employed in order to analyze the effects of finite correlation time on the long-time behavior of the phase transition between an active and an ab- sorbing state. The calculation is performed to the one-loop order. Stable fixed points of the renormalization group and their regions of stability are obtained within the three-parameter $(\epsilon,y,\eta)$- expansion. Different regimes corresponding to the rapid- change limit and frozen velocity field are discussed.

==> biblio.tex <==
%
%    SORT CITATIONS IN THE ARTICLE ACCORDING FIRST APPEARANCE - DO AT THE VERY END OF PREPARATIONS
%
\begin{thebibliography}{99}
 \bibitem{Hin06} H.~Hinrichsen, Physica A {\bf 369}, 1 (2006).
 \bibitem{Stauffer} D.~Stauffer, A.~Aharony, {\it Introduction to Percolation Theory}
     (Taylor and Francis, London, 1992).
 \bibitem{HHL08} M.~Henkel, H.~Hinrichsen, S.~L{\"u}beck, 
     {\it Non-equilibrium phase transitions: Volume 1 – Absorbing phase transitions}, 
     (Springer, Dordrecht, 2008).
 \bibitem{Schlogl} F.~Schl\"ogl, Z. Phys. {\bf 253}, 147 (1972).
 \bibitem{Grassberger82} P.~Grassberger, Z. Phys. B: Condens. Matter {\bf 47}, 365 (1982).
 \bibitem{Gribov} V.~N.~Gribov, Sov. Phys. JETP {\bf 26}, 414 (1968).    
 \bibitem{Cardy} J. L. Cardy and R. L. Sugar, \emph{ J. Phys. A} {\bf 13}, L423–L427, (1980).
 \bibitem{Hinrichsen} H.~Hinrichsen, J. Stat. Mech.: Theor. Exp. P07066 (2007).
 \bibitem{Janssen81} H.~K.~Janssen, Z. Phys. B: Condens. Matter {\bf 42}, 151 (1981).
 \bibitem{Janssen96} H.~K.~Janssen, Phys. Rev. E {\bf 55}, 6253 (1997).
 \bibitem{RRR03} P.~Rupp, R.~Richter, I.~Rehberg, Phys. Rev. E {\bf 67}, 036209 (2003).
 \bibitem{TKCS07} K.~A.~Takeuchi, M.~Kuroda, H.~Chat, M.~Sano, Phys. Rev. Lett. {\bf 99}, 234503 (2007).
 \bibitem{FGV01} G.~Falkovich, K.~Gaw\c{e}dzki, M.~Vergassola, Rev. Mod. Phys. {\bf 73}, 913 (2001). 
 \bibitem{Landau_fluid} L.~D.~Landau and E.~M.~Lifshitz, {\it Fluid Mechanics} (Pergamon Press, 1959).
 \bibitem{Frisch} U.~Frisch, {\it Turbulence: The Legacy of A. N. Kolmogorov} (Cambridge University Press, Cambridge, 1995). 
 \bibitem{Monin} A.~S.~Monin and A.~M.~Yaglom, {\it Statistical Fluid Mechanics:Vol 2}
    (MIT Press, Cambridge, 1975). 
 \bibitem{Ant99} N.~V.~Antonov, Phys. Rev. E {\bf 60}, 6691 (1999).
 \bibitem{Benzi09} R.~Benzi and D.~R.Nelson", Physica D {\bf 238}, 2003 (2009).
 \bibitem{Pig12} S.~Pigolotti and R.~Benzi and M.~H.~Jensen and D.~R.~Nelson, 
    Phys. Rev. Lett. {\bf 108}, 128102 (2012).
 \bibitem{Volk14} R.~Volk and C.~Mauger and M.~Bourgoin and C.~Cottin-Bizonne
	      and C.~Ybert and F.~Raynal, Phys. Rev. E {\bf 90}, 013027 (2014).
 \bibitem{depietro15} M.~De~Pietro and M.~A.~T.~van~Hinsberg and L.~Biferale and
	      H.~J.~H.~Clercx and P.~Perlekar and F.~Toschi, Phys. Rev. E {\bf 91}, 053002 (2015).
 \bibitem{Ant00} N.~V.~Antonov, Physica D {\bf 144}, 370 (2000).
 \bibitem{AntKap08} N.~V.~Antonov, V.~I.~Iglovikov, A.~S.~Kapustin, J. Phys. A: Math. Theor. {\bf 42}, 135001 (2008).
 \bibitem{AntKap10} N.~V.~Antonov, A.~S.~Kapustin, J. Phys. A: Math. Theor. {\bf 43}, 405001 (2010).
 \bibitem{Ant11} N.~V.~Antonov, A.~S.~Kapustin, A.~V.~Malyshev, Theor. Math. Phys. {\bf 169}, 1470 (2011).
 \bibitem{DP13} M.~Dan\v{c}o, M.~Hnati\v{c}, T.~Lu\v{c}ivjansk\'{y} and L.~Mi\v{z}i\v{s}in, Theor. Math. Phys. {\bf 176}, 898 (2013).
 \bibitem{Vasiliev} A.~N.~Vasil'ev, {\it The Field Theoretic Renormalization Group in Critical Behavior Theory and Stochastic Dynamics}
 \bibitem{JanTau04} H.~K.~Janssen, U.~C.~T{\"a}uber, Ann. Phys. {\bf 315}, 147 (2004).
 \bibitem{Doi} M.~Doi, J. Phys. A {\bf 9}, 1465 (1976); {\it ibid.} {\bf 9}, 1479 (1976).        
 \bibitem{Janssen76} H.~K.~Janssen, Z. Phys. B: Condens. Matter {\bf 23}, 377 (1976).
 \bibitem{deDom76} C.~De~Dominicis, J. Phys. Colloq. France {\bf 37}, C1-247 (1976).
 \bibitem{Janssen79} H.~K.~Janssen, {\it Dynamical Critical Phenomena and Related Topics},
    Lect. Notes Phys. {\bf 104}, (Springer, Heidelberg, 1979).
 \bibitem{Zinn} J.~Zinn-Justin, \textit{Quantum Field Theory and Critical Phenomena} (Oxford University Press, Oxford, 1989).   
 \bibitem{AdzAnt98} L.~Ts.~Adzhemyan, N.~V.~Antonov, Phys. Rev. E {\bf 58}, 7381 (1998).   
 \bibitem{Amit} D. J. Amit and V. Mart\'in-Mayor, {\it Field Theory, the Renormalization Group and Critical Phenomena}
 (World Scientific, Singapore, 2005). 
 \bibitem{Tauber2014} U.~T{\"a}uber, {\it Critical Dynamics: A Field Theory Approach to Equilibrium
 	      and Non-Equilibrium Scaling Behavior}
 	      (Cambridge University Press , New York, 2014).
 \bibitem{AAK94} L.~Ts. Adzhemyan, N.~V.~Antonov, T.~L.~Kim, Theor. Math. Phys. {\bf 100}, 1086 (1994).
 \bibitem{ABG96} N.~V.~Antonov, S.~V.~Borisenok, V.~I.~Girina, Theor. Math. Phys. {\bf 106}, 75 (1996).
 \bibitem{AV97} N.~V.~Antonov, A.~N.~Vasil'ev, Theor. Math. Phys. {\bf 110}, 97 (1997).
 \bibitem{FNS} D.~Forster, D.~R.~Nelson, M.~J.~Stephen, Phys. Rev. A {\bf 16}, 732 (1977).
 \bibitem{HH00} M.~Hnatich, J.~Honkonen, Phys. Rev. E {\bf 61}, 3904 (2000).
 \bibitem{HonKar88} J.~Honkonen and E.~Karjalainen, J. Phys. A: Math. Gen. {\bf 21}, 4217 (1988). 
 \bibitem{GV99} K.~Gaw{\c{e}}dzki, M.~Vergasssola, Physica D {\bf 138}, 63 (1999).
\end{thebibliography}
